Priority-Aware Model-Distributed Inference at Edge Networks

Distributed inference techniques can be broadly classified into data-distributed and model-distributed schemes. In data-distributed inference (DDI), each worker carries the entire Machine Learning (ML) model but processes only a subset of the data. However, feeding the data to workers results in high communication costs, especially when the data is large. An emerging paradigm is model-distributed inference (MDI), where each worker carries only a subset of ML layers. In MDI, a source device that has data processes a few layers of ML model and sends the output to a neighboring device, i.e., offloads the rest of the layers. This process ends when all layers are processed in a distributed manner. In this paper, we investigate the design and development of MDI when multiple data sources co-exist. We consider that each data source has a different importance and, hence, a priority. We formulate and solve a priority-aware model allocation optimization problem. Based on the structure of the optimal solution, we design a practical Priority-Aware Model- Distributed Inference (PA-MDI) algorithm that determines model allocation and distribution over devices by taking into account the priorities of different sources. Experiments were conducted on a real-life testbed of NVIDIA Jetson Xavier and Nano edge devices as well as in the Colosseum testbed with ResNet-50, ResNet- 56, and GPT-2 models. The experimental results show that PA-MDI performs priority-aware model allocation successfully while reducing the inference time as compared to baselines.

==> 6nodes_test.tex <==
\section{Multi-Topology and Dynamic-Topology}
\label{sec:multi-topo}
%\vspace{-7pt}
A fully connected topology, using 5 Jetson Xavier NX devices as workers, was investigated in previous tests. However, the evaluation of \ours in hardware-heterogeneous and non-fully connected scenarios remains an open question. To address this, we consider a multi-topology setup, as shown in Fig. \ref{fig:multi-topo}.

Additionally, the ability of \ours to handle mobility is tested, focusing on its performance in a dynamic topology where workers may join and leave the system over time.

\begin{figure}[htbp]
%\vspace{-5pt}
\centering
\centerline{\includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=0.48\textwidth]{figures/6-nodes-topo.png}}
\caption{Multi-Topology Test
}
\label{fig:multi-topo}
\vspace{0pt}
\end{figure}





\subsection{Setup}

The multi-topology testbed is hardware-heterogeneous, consisting of 3 Jetson Xavier NX devices and 3 Jetson Nano devices, which differ in computational level. The Jetson Nano features a less powerful CPU and smaller RAM, equipped with a 4-core ARM Cortex A57 CPU @ 1430 MHz and 4 GB of RAM. All Jetsons are connected via Wi-Fi in Ad Hoc mode, similar to the previous fully connected topology test.


The experiment uses the ResNet-50 model and a modified CIFAR-10 dataset (resized to 224x224) for deployment. Different source nodes deploy datasets with varying priorities. Workers A and D serve as source nodes, represented as larger circular symbols in Fig. \ref{fig:multi-topo}, where Worker A is a Jetson Xavier NX and Worker D is a Jetson Nano.

AR-MDI and MS-MDI are specifically designed for circular topologies. Consequently, when applied to a non-circular topology, we must select a circular chain for them. In our tests, the MDI chains chosen for AR-MDI are A: [ A, B, E, D, F, C] and D: [ D, F, C, A, B, E]. Similarly, the MDI chains chosen for MS-MDI are [ A, B, E, D, F, C]  for A and [ D, F, C, A, B, E] for D. This approach ensures compatibility of AR-MDI and MS-MDI within the non-circular topology.

\subsection{Muilt-Hop}

In this topology, multi-hop communication is enabled, allowing tasks to traverse through intermediary nodes. For instance, a task originating from node D can reach node B via node A. It is noted that in the multi-hop scenario, when each node solves the optimization problem mentioned above of \ours, the communication delay $d_{n,j}$ also incorporates the historical cumulative delays experienced as the task traverses different nodes in the network. This is because, when a task hops multiple times, the communication delays introduced by these hops must also be taken into account.


\subsection{Baselines and Performance Metric}
The baselines and performance metric remain consistent with previous tests, using AR-MDI, MS-MDI, and Local as baselines. Performance is still evaluated based on the "Average Inference Time."

\subsection{Mobility of Nodes}
To test mobility, we introduce a mechanism allowing specific nodes to join and leave the topology over time. When a mobile node leaves, it becomes unobservable to other nodes, pause communication, and keeps idle after completing current ongoing tasks. It is noted that only helper nodes may be mobile in the network, and source node remains stationary and does not leave the network.

The departure and return times of the mobile nodes are totally random and follow a Poisson distribution. Therefore, the time intervals between consecutive events of nodes leaving or returning follow an exponential distribution. In our test, the time intervals for leaving or returning are randomly generated, with an average interval configured to be 50 seconds.

PA-MDI naturally handles mobile nodes through its RTC/CTC mechanisms. When a mobile node leaves, it ceases to respond to CTC messages and receive tasks, ensuring that MDI does not terminate.

For comparison, AR-MDI and MS-MDI use a basic recovery strategy mentioned in their original papers: "wait until timeout, then bypass the leaving node." In our implementation, we adopt a more idealized recovery approach, where nodes detect departures instantaneously and bypass leaving nodes without delay, allowing MDI to continue seamlessly. This implementation grants AR-MDI and MS-MDI an advantage in dynamic topologies, meaning their real-world performance in such scenarios may be worse than our test results.


\subsection{Results}
In the first scenario of the multi-topology experiment, the topology is static with no mobile nodes. Worker A, a Jetson Xavier NX source node, hosts the "Non-Time-Sensitive" modality; while Worker D, a Jetson Nano source node, hosts the "Time-Sensitive" modality. As shown in Fig. \ref{fig:test-6nodes-static-A0-D1}, \ours algorithm significantly reduces the average inference time for "Time-Sensitive" tasks compared to the AR-MDI, MS-MDI, and Local baselines. AR-MDI and MS-MDI lack optimization for multi-source processing or different prioritizations. \ours(2,2) and \ours(4,4) both demonstrate exceptional performance and show similar results. This demonstrates that our approach can adapt effectively to different slicing policies. Compared to AR-MDI, MS-MDI, and Local, \ours reduces the average inference time for "Time-Sensitive" modalities by up to 71. 4\%, 61. 0\% and 70. 1\%, respectively. \ours also improves the inference time for "Non-Time-Sensitive" data compared to AR-MDI and MS-MDI due to its efficient resource allocation for MDI.

\begin{figure}[htbp]
%\vspace{-5pt}
\centering
\centerline{\includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=0.48\textwidth]{figures/6node-static-A0-D1.png}}
\caption{The topology is static with no mobile nodes for multi-topology test. Worker A, a Jetson Xavier NX source node, hosts the "Non-Time-Sensitive" modality; while Worker D, a Jetson Nano source node, hosts the "Time-Sensitive" modality.
}
\label{fig:test-6nodes-static-A0-D1}
\vspace{0pt}
\end{figure}


In the second scenario, we swapped the task types of source nodes A and D. Thus, Worker A, a Jetson Xavier NX source node, hosts the "Time-Sensitive" modality; while Worker D, a Jetson Nano source node, hosts the "Non-Time-Sensitive" modality. The experimental results shown in Fig. \ref{fig:test-6nodes-static-A1-D0} are similar to those observed in the first test scenario. Our method achieves a significant reduction in the average inference time for "Time-Sensitive" tasks compared to the AR-MDI, MS-MDI, and Local baselines. Likewise, \ours(2,2) and \ours(4,4) both deliver outstanding performance with comparable results. Compared to AR-MDI, MS-MDI, and Local, PA-MDI achieves reductions in the average inference time for "Time-Sensitive" modalities by up to 56.1\%, 57.8\%, and 27.1\%, respectively. It is worth noting that, in the scenario, our approach shows a comprehensive advantage over the baselines, even for all Non-Time-Sensitive tasks. This indicates that, in specific scenarios, Non-Time-Sensitive tasks can also benefit from our algorithm thanks to our efficient MDI mechanism. 


\begin{figure}[htbp]
%\vspace{-5pt}
\centering
\centerline{\includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=0.48\textwidth]{figures/6node-static-A1-D0.png}}
\caption{The topology is static with no mobile nodes for multi-topology test. Worker A, a Jetson Xavier NX source node, hosts the "Non-Time-Sensitive" modality; while Worker D, a Jetson Nano source node, hosts the "Time-Sensitive" modality.
}
\label{fig:test-6nodes-static-A1-D0}
\vspace{0pt}
\end{figure}

==> msAR-MDI.tex <==
%\vspace{-5pt}
\section{Model-Distributed Inference with Early-Exit}
\label{sec:MDI-Exit}
%\vspace{-5pt}

In this section, we present our model-distributed inference with early exit (MDI-Exit) design. We first present inference, early-exit, and offloading policies of MDI-Exit. Then, we detail data admission policies of MDI-Exit. 

\subsection{Inference, Early-Exit, and Offloading} 

%
%Our approach builds on Network Utility Maximization (NUM) \cite{neely2010stochastic}  and its solution, where each task is associated with a queue, and task scheduling decisions are made based on queue sizes. 
%\subsection{Design} 

\textbf{Inference and Early-Exit.} The first step of our MDI-Exit design is to determine when to perform inference and early-exit. Our policy is summarized in Alg. \ref{alg:Inf-Exit}. In particular, Worker $n$ checks its input queue $\Iset_n$, which stores the tasks that are supposed to be processed by Worker $n$. If there exists a task in $\Iset_n$, let us assume that this task is $\tau_k(d)$, Worker $n$ performs inference task by processing the layers in $\Lset_k$ corresponding to the task $\tau_k(d)$. After processing all the layers in  $\Lset_k$, Worker $n$ reaches the $k$th exit point. Therefore, it checks if early-exit is possible or not. The feature vector at the exit point is passed through a classifier as explained in Section \ref{sec:system} and the confidence level $C_k(d)$ is calculated according to (\ref{eq:Confidence-k}). If the confidence level $C_k(d)$ is larger than the early-exit threshold $T_e^k$, then Worker $n$ exists from the DNN model for data $A_d$ and sends the output of the classifier to the source. On the other hand, \ie if the confidence level is not reached, Worker $n$ creates a new task $\tau_{k+1}(d)$ for data $A_d$ until the $k+1$th early-exit point. Worker $n$ determines which queue the task $\tau_{k+1}(d)$ should be put according to the sizes of input and output queues. In particular, if the input queue $\Iset_n$ is empty or the size of the output queue; $O_n$ is larger than a predetermined threshold $T_O$, then the new task $\tau_{k+1}(d)$ is inserted in the input queue as it means that local processing of tasks at Worker $n$ is faster. Otherwise, it is inserted in the output queue as it means that offloading is faster. 




\begin{algorithm}[t!]
\caption{Inference and Early-Exit of MDI-Exit at Worker $n$.}\label{alg:Inf-Exit}
\begin{algorithmic}[1]
\STATE \textbf{Input:}  Early-exit threshold $T_e^k$, $\forall k$. Output queue threshold $T_O$. Input queue $\Iset_n$. Output queue $\Oset_n$.
\WHILE{There exists a task in $\Iset_n$}
\STATE Process the head-of-line task $\tau_k(d)$.
\STATE Calculate the confidence level  $C^k(d)$ according to (\ref{eq:Confidence-k}). 
\IF{$C^k(d) > T_e^k$}
\STATE Early exit and send the output of the classifier ($b_l^k(d)$) to the source. 
\ELSE
\IF{The input queue $\Iset_n$ is empty OR $O_n > T_O$ }
\STATE Insert the new task $\tau_{k+1}(d)$ to $\Iset_n$.
\ELSE
\STATE Insert the new task to $\Oset_n$.
\ENDIF
\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}


\textbf{Offloading.} The next step in our MDI-Exit design is offloading. Worker $n$ offloads the tasks in its output queue to its one-hop neighbors. The task offloading policy from Worker $n$ to Worker $m$, considering that they are one-hop neighbors, is summarized in Alg. \ref{alg:Offloading} and will be detailed next. 

If there exists a task in the output queue $\Oset_n$, Worker $n$ explores the opportunities of offloading its tasks. Worker $n$ periodically learns from its one-hop neighbor Worker $m$ its input queue size $I_m$, per task computing delay $\Gamma_m$\footnote{We note that exit points could be arranged in a way that each task has a similar amount of computation requirements. Thus, $\Gamma_m$ can be measured independently from the identities of the tasks.} as well as transmission delay $D_{nm}$ between Workers $n$ and $m$. Worker $n$ runs Alg. \ref{alg:Offloading} for each of its one-hop neighbors. If the output queue size of Worker $n$ is larger than the input queue size of Queue $m$, \ie $O_n > I_m$ is satisfied; Worker $n$ concludes that its neighbor Worker $m$ is in a better state than itself in terms of processing tasks. Next, Worker $n$ compares the task completion delays. 

If a task at Worker $n$ is processed locally, it needs to wait so that all the tasks in the input queue are processed, so its waiting time is $I_n\Gamma_n$. If it is offloaded to Worker $m$, it needs to be transmitted and wait for all the tasks in the input queue of Worker $m$, so its waiting time is $D_{nm} + I_m \Gamma_m$. Thus, Worker $n$ compares these delays. If $I_n\Gamma_n > D_{nm} + I_m \Gamma_m$, the task is offloaded to Worker $m$ (line 3). Otherwise, the task is offloaded to Worker $m$ with  probability $\min\{\frac{I_n\Gamma_n }{D_{nm} + I_m\Gamma_m}, 1\}$ (line 5). The reason behind the probabilistic offloading is to utilize resources effectively. Even if offloading a task introduces a higher delay, offloading may still 
be good, considering that $O_n > I_m$ and the probabilistic transmission occur when local processing and offloading delays are on similar orders. 


\begin{algorithm}[t!]
\caption{Offloading from Worker $n$ to $m$.}\label{alg:Offloading}
\begin{algorithmic}[1]
\WHILE{There exists a task in $\Oset_n$}
\IF{$O_n > I_m$ AND $I_n\Gamma_n  >  D_{n,m} + I_m \Gamma_m$} 
\STATE Offload the head-of-line task from $\Oset_n$ to Worker $m$.
\ELSIF{$O_n > I_m$}
\STATE Offload the head-of-line task from $\Oset_n$ to Worker $m$ with probability $\min\{\frac{I_n\Gamma_n }{D_{nm} + I_m\Gamma_m}, 1\}$.
\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}


\subsection{Data Admission Policies} Suppose that Worker $n$ is the source. It may already have the data or collect the data from the environment according to some distribution. The question in this context is how to guarantee that all the data at the source is admitted and processed for DNN inference. We consider two scenarios: (i) Data arrival rate is adapted assuming that early-exit threshold is fixed. (ii) Early-exit threshold is adapted assuming that data arrival follows a general distribution. 

%Data rate follows a Poisson distribution and early-exit confidence threshold is adapted to admit all the traffic. 

\textbf{Data Arrival Rate Adaptation.} We first fix the early-exit confidence threshold $T_e^k$ for all tasks. Our goal is to adapt the arrival rate of the data that is collected/generated at the source. In other words, the source worker collects/generates data by following the ``inference rate'' that MDI-Exit imposes.  This scenario suits well for applications where a certain inference accuracy (confidence threshold) is needed while data arrival rate can be adapted. 

Our policy determines the interarrival time of data $\mu$ at the source. Our approach is inspired by congestion control mechanisms of delay-based TCP algorithms, \eg TCP Vegas. Let us assume that the source worker is Worker $n$. Our algorithm summarized in Alg. \ref{alg:interarrivalTime} uses the queue size information to determine the interarrival time $\mu$ at the source. In particular, if $I_n + O_n < T_{Q1}$, then the interarrival time $\mu$ is reduced according to line 3 to increase the data rate, where $\alpha$ is a predetermined constant between $0$ and $1$. The data rate is increased (interarrival time is reduced) in this case, because the number of tasks in input and output queues is very low, which means that the MDI-Exit system can handle more data. If $I_n + O_n > T_{Q1}$ but $I_n + O_n < T_{Q2}$, interarrival time is reduced according to line 5, but not as dramatically as line 3, because $\alpha > \beta$. Finally, if $I_n + O_n > T_{Q2}$, interarrival time is increased according to line 7 to decrease the data rate because queues are highly occupied. The data rate should be reduced so that the queue sizes remain bounded. We note that after every update on interarrival time $\mu$, the algorithm sleeps for $s$ seconds to give some time to queues to update their states. Alg. \ref{alg:interarrivalTime} runs again after the sleep time is over. 


\begin{algorithm}[t!]
\caption{Data Interarrival Time Adaptation at Source.}\label{alg:interarrivalTime}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Assume source worker is Worker $n$. Input queue size at the source $I_n$. Output queue size at the source $O_n$. Constants $\alpha$, $\beta$, and $\zeta$ between 0 and 1 and $\alpha > \beta$. Queue thresholds $T_{Q1}$ and $T_{Q2}$, where $T_{Q1} \leq T_{Q2}$. Sleep duration $s$. 
\IF{$I_n+O_n < T_{Q1}$}
\STATE $\mu = \mu - \alpha \mu$. Sleep for $s$ seconds. 
\ELSIF{$I_n+O_n > T_{Q1}$ AND $I_n+O_n < T_{Q2}$}
\STATE $\mu = \mu - \beta \mu$. Sleep for $s$ seconds. 
\ELSIF{$I_n+O_n > T_{Q2}$}
\STATE $\mu = \mu + \zeta \mu$. Sleep for $s$ seconds. 
\ENDIF
\end{algorithmic}
\end{algorithm}


\textbf{Early-Exit Threshold Adaptation.} In this setup, we consider that all the traffic arriving to the source worker should be processed, which can only be feasible with reduced accuracy. In other words, if the data rate is too high, more early-exits should happen (lower early-exit threshold, hence lower accuracy) to accommodate all the data. Otherwise, early-exit threshold (hence accuracy) can be increased as less data needs to be processed. Our approach, summarized in Alg. \ref{alg:ConfLevel}, follows a similar idea in Alg. \ref{alg:interarrivalTime}. In particular, if queues are not heavily occupied, the early-exit threshold is increased (lines 3 and 5). We note that the largest value of the early-exit threshold could be 1 due to the normalization in (\ref{eq:Confidence-k}), so we use $T_e = \min\{1, T_e + \alpha T_e\}$ and $T_e = \min\{1, T_e + \beta T_e\}$ in lines 3 and 5 respectively. On the the other hand, if queue occupancy is high (line 6), then the early-exit threshold is reduced (line 7), noting that early-exit threshold cannot be less than the minimum early-exit threshold $T_e^{\min}$ that we set. 



\begin{algorithm}[t!]
\caption{Confidence Level Adaptation at Worker $n$.}\label{alg:ConfLevel}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Input queue size  $I_n$. Output queue size $O_n$. Constants $\alpha$, $\beta$, and $\zeta$ between 0 and 1 and $\alpha > \beta$. Queue thresholds $T_{Q1}$ and $T_{Q2}$, where $T_{Q1} \leq T_{Q2}$. Sleep duration $s$. Current confidence level $T_e$.  Minimum confidence level $T_e^{\min} > 0$.
\IF{$I_n+O_n < T_{Q1}$}
\STATE $T_e = \min\{1, T_e + \alpha T_e\}$. Sleep for $s$ seconds. 
\ELSIF{$I_n+O_n > T_{Q1}$ AND $I_n+O_n < T_{Q2}$}
\STATE $T_e = \min\{1, T_e + \beta T_e\}$. Sleep for $s$ seconds. 
\ELSIF{$I_n+O_n > T_{Q2}$}
\STATE $T_e = \max\{T_e^{\min}, T_e - \zeta T_e\}$. Sleep for $s$ seconds. 
\ENDIF
\STATE $T_e^k  \leftarrow T$, $\forall k$. 
\end{algorithmic}
\end{algorithm}







% \begin{figure}[t!]
% %\vspace{-5pt}
%     \centering
%     \scalebox{0.48}{
%     \includegraphics{figures/MS-AR-MDI-Algorithm.eps}}
%     \vspace{-15pt}
%     \caption{Queue constructions and task scheduling decisions in an example topology of Fig. \ref{fig:MS-MDI}. We focus on the operations of worker 1, \ie $\eta_1$, in this figure.}
%     \label{fig:MS-MDI-queue}
%     \vspace{-10pt}
% \end{figure}

% \textbf{Queue Construction.} Each source worker $\eta_i$ constructs a queue $q_l^i$, which stores data that are supposed to be processed locally at worker $\eta_i$. In other words, the data in $q_l^i$ is not processed in a distributed manner, but locally at $\eta_i$. Each worker (either a source or not) $\eta_n$, $n \in \Nset$ constructs $|\Sset|$ queues $q_n^i$ for each source node $i \in \Sset$. The queue $q_n^i$ stores data or activation vectors that node $\eta_n$ is supposed to process for source node $\eta_i$ in a distributed manner. Let us consider the example topology in Fig. \ref{fig:MS-MDI} again in Fig. \ref{fig:MS-MDI-queue} and focus on $\eta_1$. The source device $\eta_1$ constructs three queues; (i) $q_l^1$ for processing its own data locally, (ii) $q_1^1$ for processing its own data via MDI, and (iii) $q_1^3$ for processing $\eta_3$'s data via MDI. 

% \textbf{Data arrival in sources.} In source worker $\eta_i$, if data is collected or arrives according to Poisson distribution, such data is inserted in a reservoir queue $\mu_i$. Then, at time slot $t$, fixed amount of data is taken from $\mu_i$, and inserted in a queue that satisfies $\min \{q_l^i(t), q_i^i(t)\}$. We note that $q_l^i(t)$ represents local processing (inference) queue at time $t$, while $q_i^i(t)$ corresponds to the distributed processing queue. Our design of MS-MDI selects the smallest queue among $q_l^i(t)$ and $q_i^i(t)$ for inserting new data arrivals, because the smallest queue likely corresponds to the policy, \ie either local or MDI, that processes data faster. For example, $\eta_1$ in Fig. \ref{fig:MS-MDI-queue} checks $\min\{q_l^1, q_1^1\}$ and inserts the new arrivals to the smallest queue. 


% \begin{figure*}[t!]
% \centering
% \subfigure[Two-worker]{ \scalebox{.28}{\includegraphics{figures/2worker-grids.eps}} } 
% \subfigure[Three-worker]{ \scalebox{.28}{\includegraphics{figures/3worker-grids.eps}} } 
% \subfigure[Increasing number of workers]{ \scalebox{.38}{\includegraphics{figures/NumberOfWorkersVSavgProcessingTime.eps}} } 
% \vspace{-8pt}
% \caption{Inference/processing time versus the number of images in a (a) two worker setup, and (b) three worker setup. (c) Inference/processing time versus the number of workers. Two out of all workers are source workers in all experiments. }
% \vspace{-10pt}
% \label{fig:all-results}
% \end{figure*}


% \textbf{Selection of queues for inference.} At slot $t$, each node $\eta_n$ decides which data should be processed according to 
% \begin{align} \label{eq:policy2}
%     \max \{ q_l^n(t), \max_{j \in \Sset} \{ q_n^j(t) - q_{(n+1)\%N}^j(t) \} \},
% \end{align} where $q_n^j(t) = -M$ if $n \notin \Sset$ and $M$ is a large positive constant. If $q_l^n(t)$ is the maximum term in (\ref{eq:policy2}), data from $q_l^n(t)$ is taken and processed locally at node $n$. Otherwise, \ie if $\max_{\forall j \in \Sset} \{ q_n^j(t) - q_{(n+1)\%N}^j(t) \} $ is the maximum term, $z = \arg \max_{\forall j \in \Sset} \{ q_n^j(t) - q_{(n+1)\%N}^j(t) \} $ is determined. Then, data from $q_n^z(t)$ is processed at worker $\eta_n$ according to MDI. The output of the process, \ie the activation vector of the last layer $a_{l_n^z}^z(k)$ is sent to the next node $\eta_{(n+1)\%N}$. Let us consider $\eta_1$ in Fig. \ref{fig:MS-MDI-queue} again. If the maximum term of $\max\{q_l^1, \max_{i \in {1,3}}\{q_1^i - q_2^i\}\}$ is $q_l^1$, $\eta_1$'s data is processed locally at $\eta_1$. If the maximum term is  $q_1^i - q_2^i$, $i \in \{1,3\}$ then $\eta_i$'s data is processed partially, and the activation vector of the last layer is transmitted to $\eta_2$. We note that activation vectors coming from $\eta_4$ are an input to $q_1^3$. The rationale behind selecting the largest queue is to ramp up the speed of data processing for large queues. %This approach is based on the solution of NUM problem as shown in \cite{ExtendedThis}. 

% %stabilizes the queues and leads to utility optimal operation \cite{neely2010stochastic}. 


% %$\max\{q_l^1, \max_{i \in {1,3}}\{q_1^i - q_2^i\}\}$

% %If $z \neq n$, then data (which is typically activation vector) is sent to  


% % \begin{theorem} \label{th:stability}
% % If XXXXXXXXXXXXXXXXXXXXXX.

% % \end{theorem}

% %\subsection{Analysis}


